Attentive Temporal Pooling for Conformer-based Streaming Language Identification in Long-form Speech

In this paper, we introduce a novel language identification system based on conformer layers. We propose an attentive temporal pooling mechanism to allow the model to carry information in long-form audio via a recurrent form, such that the inference can be performed in a streaming fashion. Additionally, we investigate two domain adaptation approaches to allow adapting an existing language identification model without retraining the model parameters for a new domain. We perform a comparative study of different model topologies under different constraints of model size, and find that conformer-based models significantly outperform LSTM and transformer based models. Our experiments also show that attentive temporal pooling and domain adaptation improve model accuracy.

==> confidence.tex <==
\subsection{Confidence modeling}
\label{sec:confidence}

\Jason{1/20/2022: For this section... I think there are really two problems we need to address here. (1) The first is that we need to perform confidence score re-calibration' because we train an end-to-end neural network model that has many free parameters and gives optimistic 'probability' scores for the data. We need to re-calibrate using various features/scores with a small model to produce reliable confidence estimates. (2) Are we doing language diarization? We are giving examples that lend to language diarization and not language ID. (e.g. comparing $\mat{p}_a$ and $\mat{p}_b$.) If we are doing language diarization, we should propose a cost function that reflects the overall cost of the language diarization. i.e. It would include the cost of outputting false language switches or missing language switches. If it is within scope, we could put together a cost function similar to what is done with NIST (this would add to the novelty). i.e. sum of weighted cost of false change points and missed change points.}

In many applications of LangID, knowing the top hypothesized language that has the highest probability is insufficient. The confidence of this top hypothesis is also critical for the application to function well.

For example, in multilingual conversations where people speak different languages within a single speech session, LangID predictions can be used to code switch ASR models in different languages to produce multilingual transcription. This process is also referred to as ``language diarization''~\cite{lyu2013language}. \Jason{FA and FR is a little vague in the following sentence. I think we want to talk about it in the context of detecting/missing the language change point. The way it is currently written suggests it may be accepting/rejecting the specific candidate language for a particular segment.} For this kind of application, users are usually more tolerant over false rejects (FR) than false accepts (FA) --- \Jason{Let's make the following sentence more concise... wordy.} mistakenly switching the language for a monolingual utterance is considered a much worse user experience than failing or being slow to switch the language in a multilingual utterance.

To address this, a confidence model could be very helpful such that code switch is only triggered when the LangID prediction has a very high confidence. The simplest form of confidence is to directly use the output probability of the top language $\max(\mat{p}_t)$ as the confidence. \Jason{Why is the original probability not a high quality confidence? - we did not explain this.} However, this simple approach is usually insufficient when high-quality confidence is needed. For example, consider two probability distributions:
\begin{eqnarray}
    \mat{p}_a &=& [0.5, 0.49, 0.01], \\
    \mat{p}_b &=& [0.5, 0.25, 0.25] .
\end{eqnarray}
\Jason{Based on our previous discussions one perspective suggests we can be more confident in the top language with $\mat{p}_b$. But what about the following...
\begin{eqnarray}
    \mat{p}_a &=& [0.5, 0.49, 0.01], \\
    \mat{p}_b &=& [0.48, 0.26, 0.26] .
\end{eqnarray}
Which result gives us the best chance of guessing the language correctly?
}


\Jason{We need to address this paragraph below. By definition, the probability of the first language being correct is the same, whether it is $\mat{p}_a$ or $\mat{p}_b$. i.e. For the first language, either way we have a 50\% chance of being wrong. For language diarization, we may have false code switch problems with $\mat{p}_a$ versus $\mat{p}_b$... but this is a different question. We need to think about how we frame this section. Are we doing language identification or language diarization? (The title says language identification.)}
While the probability of the first language being the top language is 0.5 for both $\mat{p}_a$ and $\mat{p}_b$, we are more confident about $\mat{p}_b$, as in $\mat{p}_a$ the probability of the second language is very close to the probability of the first language.

In modern speech systems, a popular approach is to use an additional model to estimate the confidence of the output from the end-to-end trained neural network~\cite{jiang2005confidence,wessel2001confidence,li2021confidence}.
Here we propose a linear confidence model that is only based on the LangID outputs.
Given an existing LangID model, assume we run this model on a training utterance, and we get the output as a probability distribution $\mat{p}_t \in [0,1]^K$ over $K$ candidate languages at every time step $t$. We define four features based on the sequence $(\mat{p}_1, \cdots, \mat{p}_t)$:
\Jason{It would be interesting to understand the strength of contribution of each of these features.}
\begin{enumerate}
    \item The \textbf{probability} of the top language: $c_{1,t}=\max(\mat{p}_t)$;
    \item The \textbf{probability delta} between the top language and the second-best language: $c_{2,t}=\max(\mat{p}_t)-\max(\mat{p}_t \setminus c_{1,t})$;
    \item The \textbf{negentropy} of the distribution: $c_{3,t}=\ln(K)-\text{entropy}(\mat{p}_t)$;
    \item The \textbf{continuity} of predictions, which is defined as the number of consecutive predictions whose top language is the same as time $t$. This feature is denoted as $c_{4,t}$, which must be a positive integer.
\end{enumerate}

We define the final confidence score $C_t \in (0,1)$ as:
\begin{eqnarray}
    \label{eq:conf}
    C_t &=& P(y=\arg\max (\mat{p}_t) | \mat{p}_1, \cdots , \mat{p}_t) \\
    &=& \text{sigmoid} (\sum_{i=1}^4 \alpha_i \cdot c_{i,t} + \beta ), 
\end{eqnarray}
where $y$ is the ground truth language index, and $\{\alpha_1,\cdots,\alpha_4,\beta\}$ are five parameters to be trained.

Given a dev-set of $N$ utterances, for each utterance $j$, we know whether the top language predicted by the LangID model at time $t$ is correct or not, which can be represented by
\begin{eqnarray}
    z_t^{(j)} &=& \delta(y^{(j)}=\arg\max (\mat{p}_t)^{(j)}) \\ 
    &\in& \{0,1\}.
\end{eqnarray}
 Thus we can train the parameters $\{\alpha_1,\cdots,\alpha_4,\beta\}$ on this dev-set using logistic regression.
Once we have trained the confidence model, we can calibrate the threshold $\tau$ for the confidence based on the detection error tradeoff (DET) curve on this dev-set.
